Two Sides of the Same Coin: Learning the Backdoor to Remove the Backdoor

The community has recently developed various training-time defenses to counter neural backdoors introduced through data poisoning. In light of the observation that a model learns poisonous samples responsible for the backdoor easier than benign samples, these approaches either use a fixed threshold of the training loss for splitting or iteratively learn a reference model as an oracle for identifying benign samples. In particular, the latter has proven effective for anti-backdoor learning. Our method, HARVEY, leverages a similar yet crucially different technique: learning an oracle for poisonous rather than benign samples. Learning a backdoored reference model is significantly easier than learning a reference model on benign data. Consequently, we can identify poisonous samples much more accurately than related work identifies benign samples. This crucial difference enables near-perfect backdoor removal as we demonstrate in our evaluation. HARVEY substantially outperforms related approaches across attack types, datasets, and architectures, lowering the attack success rate to the very minimum at a negligible loss in natural accuracy. The figure below shows an overview of our methods working principle.

==> checklist.tex <==
\begin{enumerate}
	\item This paper:
	
	\begin{itemize}
		\item Includes a conceptual outline and/or pseudocode description of AI methods introduced \answerYes%(yes/partial/no/NA)
		
		\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results \answerYes%(yes/no)
		
		\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper \answerYes%(yes/no)
	\end{itemize}

	\item Does this paper make theoretical contributions? \answerNo%(yes/no)
	
	\iffalse
	\noindent
	If yes, please complete the list below.
	
	\begin{itemize}
		\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
		
		\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
		
		\item Proofs of all novel claims are included. (yes/partial/no)
		
		\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
		
		\item Appropriate citations to theoretical tools used are given. (yes/partial/no)
		
		\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
		
		\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
	\end{itemize}
	\fi
	
	\item Does this paper rely on one or more datasets? \answerYes%(yes/no)
	
	\iftrue
	\noindent
	If yes, please complete the list below.
	
	\begin{itemize}
		\item A motivation is given for why the experiments are conducted on the selected datasets \answerYes%(yes/partial/no/NA)
		
		\item All novel datasets introduced in this paper are included in a data appendix. \answerNA%(yes/partial/no/NA)
		
		\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerNA%(yes/partial/no/NA)
		
		\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \answerYes%(yes/no/NA)
		
		\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \answerYes%(yes/partial/no/NA)
		
		\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \answerNA%(yes/partial/no/NA)
	\end{itemize}
	\fi
	
	\item Does this paper include computational experiments? \answerYes%(yes/no)
	
	\iftrue
	If yes, please complete the list below.
	
	\begin{itemize}
		\item Any code required for pre-processing data is included in the appendix. \answerYes%(yes/partial/no).
		
		\item All source code required for conducting and analyzing the experiments is included in a code appendix. \answerYes%(yes/partial/no)
		
		\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes%(yes/partial/no)
		
		\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from \answerNo%(yes/partial/no)
		
		\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \answerNo%(yes/partial/no/NA)
		
		\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \answerYes%(yes/partial/no)
		
		\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \answerYes%(yes/partial/no)
		
		\item This paper states the number of algorithm runs used to compute each reported result. \answerNo%(yes/no)
		
		\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \answerYes%(yes/no)
		
		\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \answerYes%(yes/partial/no)
		
		\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \answerYes%(yes/partial/no/NA)
		
		\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \answerYes%(yes/partial/no/NA)
	\end{itemize}
	\fi
\end{enumerate}


==> tables/adapt-ratios-wrn.tex <==
\begin{adapttable}{\columnwidth}
%	\num{10}
%	& 	& 
%	& 	& 
%	& 	& 
%	& 	& 
%	& 	& 
%	\\
	\num{20}
	& 90.16	& 1.40
	& 89.07	& 0.80
	& 88.21	& 1.40 
	& 88.56	& 0.47
	& 87.84	& 1.62
	\\
	\num{30}
	& 90.05	& 1.41
	& 88.37	& 0.97
	& 86.43	& 0.74
	& 90.23	& 1.63
	& 86.07	& 2.65
	\\
	\num{40}
	& 83.52	& 0.03
	& 85.67	& 0.84
	& 84.24	& 1.03
	& 89.95	& 1.33
	& 85.32	& 1.86
	\\
	\num{50}
	& 82.67	& 0.00
	& 82.53	& 0.00
	& 82.95	& 0.00
	& 87.85	& 0.67
	& 84.28	& 1.17
	\\
	\bottomrule
\end{adapttable}

==> tables/adapt-ratios.tex <==
\begin{adapttable}{\columnwidth}
%	\num{10}
%	& 93.81	& 0.11
%	& 92.36	& 0.08
%	& 94.21	& 0.10
%	& 94.44	& 0.09
%	& 93.05	& 1.02
%	\\
	\num{20}
	& 93.09	& 0.23
	& 92.27	& 0.16
	& 92.15	& 0.38
	& 93.50	& 0.31
	& 93.04	& 1.34
	\\
	\num{30}
	& 92.46	& 0.07
	& 92.53	& 0.19
	& 91.28	& 0.50
	& 93.73	& 1.79
	& 91.18	& 1.95
	\\
	\num{40}
	& 91.17	& 0.00
	& 91.00	& 0.32
	& 91.34	& 0.88
	& 92.36	& 0.89
	& 89.94	& 0.44
	\\
	\num{50}
	& 89.92	& 0.00
	& 91.06	& 0.60
	& 89.93	& 0.48
	& 89.03	& 1.89
	& 89.79	& 0.51
	\\
	\bottomrule
\end{adapttable}

==> tables/dduplicate-wrn.tex <==
\begin{dduptable}{\columnwidth}
	& \multirow{6}{*}{~\poisonTarget $=$ class 0}
	& \badnets	& 89.98	& 1.13	& 86.31	& 99.86	& 92.59
	\\
	&
	& \trojan 	& 89.82	& 0.87	& 82.46	& 99.76	& 90.29
	\\
	&
	& \blend	& 88.14	& 1.57	& 66.55	& 96.48	& 78.77
	\\
	&
	& \clb		& 84.00	& 0.96	& 41.98	& 99.28	& 59.01 
	\\
	&
	& \iab		& 86.64	& 1.62	& 61.30	& 95.92	& 74.80
	\\
	&
	& \wanet	& 88.20	& 1.73	& 45.37	& 91.88	& 60.74
	\\ 
	\midrule
	%
	& \multirow{6}{*}{\makecell{\poisonTarget $\neq$ class 0\\(\poisonTarget $=$ class 1)}}
	& \badnets	& 85.46	& 0.86	& 61.79	& 99.92	& 76.36 
	\\
	&
	& \trojan	& 85.13	& 0.27	& 59.95	& 99.84	& 74.92
	\\
	&
	& \blend	& 84.43	& 1.03	& 50.45	& 98.88	& 66.82
	\\
	&
	& \clb		& 83.21	& 2.18	& 40.66	& 98.16	& 57.50
	\\
	&
	& \iab		& 84.96 & 1.77	& 53.87 & 96.08	& 69.04
	\\
	&
	& \wanet	& 83.16	& 2.74	& 37.87	& 87.10	& 52.79
	\\
	\bottomrule
\end{dduptable}

==> tables/mean-std.tex <==
%\newcommand{\meanstdreader}[3]{%
%	\csvreader[
%	head to column names,
%	filter = \equal{\dataset}{#1} \and \equal{\arch}{#2} \and 
%	\equal{\attack}{#3},
%%	late after line=\\,
%	]%
%	{res/main_results_meanstd.csv}%
%	{}
%	{	
%		& \noacctxt
%		& \noasrtxt
%		& \ouraccmean
%		& \ouraccstd
%		& \ourasrmean
%		& \ourasrstd
%		&
%	}
%}
%
%%{\meanstdreader{cifarten}{resnetS}{badnets}}
%
%\begin{meanstdtable}{\columnwidth}
%	\multirow{8}{*}{\rotatebox{90}{\resnet{18}}}
%	& \badnets	\meanstdreader{cifarten}{resnetS}{badnets}
%	\\
%	& \trojan	\meanstdreader{cifarten}{resnetS}{trojan}
%	\\
%	& \blend	\meanstdreader{cifarten}{resnetS}{blend}
%	\\
%	& \clb		\meanstdreader{cifarten}{resnetS}{clb}
%	\\
%	& \wanet	\meanstdreader{cifarten}{resnetS}{wanet}
%	\\ \cmidrule{2-8}
%	& \iab		\meanstdreader{cifarten}{resnetS}{iab}
%	\\
%	& \ssba	\meanstdreader{cifarten}{resnetS}{ssba}
%%	\\
%%	& \sleepagent	\meanstdreader{cifarten}{resnetS}{sleepagent}
%	\\ \midrule
%	\multirow{8}{*}{\rotatebox{90}{\wrn}}
%	& \badnets	\meanstdreader{cifarten}{wrn}{badnets}
%	\\
%	& \trojan	\meanstdreader{cifarten}{wrn}{trojan}
%	\\
%	& \blend	\meanstdreader{cifarten}{wrn}{blend}
%	\\
%	& \clb		\meanstdreader{cifarten}{wrn}{clb}
%	\\
%	& \wanet	\meanstdreader{cifarten}{wrn}{wanet}
%	\\ \cmidrule{2-8}
%	& \iab		\meanstdreader{cifarten}{wrn}{iab}
%	\\
%	& \ssba	\meanstdreader{cifarten}{wrn}{ssba}
%%	\\
%%	& \sleepagent	\meanstdreader{cifarten}{wrn}{sleepagent}
%	\\ \bottomrule
%\end{meanstdtable}

\newcommand{\meanstdreader}[3]{%
	\csvreader[
	head to column names,
	filter = \equal{\dataset}{#1} \and \equal{\arch}{#2} \and 
	\equal{\attack}{#3},
	%	late after line=\\,
	]%
	{res/main_results_meanstd.csv}%
	{}
	{	
		& \ouraccmean
		& \ouraccstd
		& \ourasrmean
		& \ourasrstd
	}
}

%{\meanstdreader{cifarten}{resnetS}{badnets}}

\begin{meanstdtableshort}{\columnwidth}
	\badnets
	\meanstdreader{cifarten}{resnetS}{badnets}
	\meanstdreader{cifarten}{wrn}{badnets}
	\\
	\trojan
	\meanstdreader{cifarten}{resnetS}{trojan}
	\meanstdreader{cifarten}{wrn}{trojan}
	\\
	\blend
	\meanstdreader{cifarten}{resnetS}{blend}
	\meanstdreader{cifarten}{wrn}{blend}
	\\
	\clb
	\meanstdreader{cifarten}{resnetS}{clb}
	\meanstdreader{cifarten}{wrn}{clb}
	\\
	\iab
	\meanstdreader{cifarten}{resnetS}{iab}
	\meanstdreader{cifarten}{wrn}{iab}
	\\
	\wanet
	\meanstdreader{cifarten}{resnetS}{wanet}
	\meanstdreader{cifarten}{wrn}{wanet}
%	\\
%	\ssba
%	\meanstdreader{cifarten}{resnetS}{ssba}
%	\meanstdreader{cifarten}{wrn}{ssba}
	\\ \bottomrule
\end{meanstdtableshort}

==> tables/smallarch.tex <==
\begin{smallarchtable}{\columnwidth}
%	\multirow{6}{*}{\cifar{10}}
	\badnets	& 95.50	& 0.59	& 93.75	& 98.14	& 95.80	& 0.21
	\\
	\trojan 	& 95.25	& 0.50	& 96.24	& 99.80	& 97.99	& 0.02
	\\
	\blend		& 94.22	& 1.18	& 80.00	& 94.30	& 86.56	& 0.65
	\\
	\clb		& 93.57	& 0.05	& 100.00& 100.00& 100.00	& 0.00
	\\
	\iab		& 94.04	& 0.24	& 77.89	& 98.50	& 86.99	& 0.17
	\\
	\wanet		& 93.10	& 1.28	& 68.94	& 90.90	& 78.41	& 1.05
	\\ 
%	\midrule
%	%
%	\multirow{6}{*}{\gtsrb}
%	& \badnets	& 89.01	& 0.06	& 65.27	& 99.60	& 78.86 
%	\\
%	& \trojan	& 89.04	& 0.37	& 63.53	& 94.26	& 75.90
%	\\
%	& \blend	& 87.44	& 0.10	& 61.81	& 96.66	& 75.40
%	\\
%	& \clb		& 89.70	& 0.00	& 57.47	& 100.00& 72.99
%	\\
%	& \iab		& 90.02	& 0.04	& 69.60	& 96.12	& 80.74
%	\\
%	& \wanet	& 86.07	& 0.32	& 50.13	& 79.36	& 61.44
%	\\
	\bottomrule
\end{smallarchtable}
